What's in the Image? Explorable Decoding of Compressed Images

The ever-growing amounts of visual contents captured on a daily basis necessitate the use of lossy compression methods in order to save storage space and transmission bandwidth. While extensive research efforts are devoted to improving compression techniques, every method inevitably discards information. Especially at low bit rates, this information often corresponds to semantically meaningful visual cues, so that decompression involves significant ambiguity. In spite of this fact, existing decompression algorithms typically produce only a single output, and do not allow the viewer to explore the set of images that map to the given compressed code. In this work we propose the first image decompression method to facilitate user-exploration of the diverse set of natural images that could have given rise to the compressed input code, thus granting users the ability to determine what could and what could not have been there in the original scene. Specifically, we develop a novel deep-network based decoder architecture for the ubiquitous JPEG standard, which allows traversing the set of decompressed images that are consistent with the compressed JPEG file. To allow for simple user interaction, we develop a graphical user interface comprising several intuitive exploration tools, including an automatic tool for examining specific solutions of interest. We exemplify our framework on graphical, medical and forensic use cases, demonstrating its wide range of potential applications.

==> app_fig_editing_dunes.tex <==
\begin{figure}[t]
\centering
% \includegraphics[width=\columnwidth]{images/}
\vspace{-18pt}\caption{\label{fig:editing_dunes}\textbf{The making of Fig.~\ref{fig:dunes}.}}
\end{figure}

==> broader_impact.tex <==
\section*{Broader Impact}
Despite progress in compression algorithms, JPEG is still the most widely used image format, with billions of JPEG images produced on a daily basis. From photo albums to important sports or political events, JPEG images document the personal and collective experiences of many. 
Unfortunately, JPEG photos are not completely loyal to the scene they capture, as small and faint details are often lost in the compression process. When looking at such JPEG images (decompressed with a regular JPEG decoder), it is easy to tell that the quality in a certain region is not good enough. However, it is currently extremely difficult, if not impossible, to understand \emph{what could and what could not have been there} in the original scene. Our method is the first to grant users the possibility of doing that.

We believe that our explorable decoding framework has the potential to see widespread use. One could envision integrating it into photo viewers and web browsers, from smartphones to desktop computers, as well as exploiting it in medicine and forensics.

A natural concern is the potential misuse of such technology. Visual contents could be edited to depict a misleading picture. However, it is important to stress that as opposed to existing editing software, our approach only allows making edits that are consistent with the JPEG file. This places a stringent constraint on the possible outputs that one could generate.

%It therefore seems that the merits of our approach outweigh the minor risks associated with generating ``fake news''.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> temp_tools_description.tex <==
Tools operating on image patches (rather than directly on the image itself) use partially overlapping $6\times6$ patches. The degree of overlap varies, and indicated separately for each tool.

\subsection{Variance Manipulation}
This set of tools operates by manipulating the local variance of all partially overlapping image patches in the selected region. We employ objective function $f(\cdot)=(\text{Var}(\cdot)-c)^2$,  and optimize over $z$ to increase or decrease the local, per-patch variance to a desired value $c$, that can be set relative to the local variance of the current output image.by a pre-determined given user value.
\paragraph{Signal magnitude manipulation}
A variant of this tool preserves patches' structures and only manipulates the magnitude of their signal, after removing their mean values. This variant operates on less patches, by sub-sampling overlapping patches using a 4 rows stride.
\subsection{Encouraging Piece-wise Smoothness}
This tool acts by minimizing the total variations (TV) in a user-marked region: $f(\cdot)=\text{TV}(\cdot)$. In particular, $f(\cdot)$ is the sum of absolute differences between each pixel in the region and its $8$ neighboring pixels.
\subsection{Graphical User Input}\label{sec:graphical_input}
Our GUI constitutes a large set of Microsoft-Paint-like tools, allowing a user to impose a graphical input on the output image. These include pen and straight line tools (with adjustable line width), as well as polygon, square and circle drawing tools. Scribbling color can be chosen manually or sampled from any given image (including the edited one). Unlike in \cite{bahat2019explorable_sr}, the scribble itself is imposed in a consistency preserving manner, by projecting the scribbled region onto the set of images that are consistent with the compressed code $x_Q$. Namely, each block of DCT coefficients $X^{\text{scribbled}}_D$ of the scribbled region is modified into
\begin{equation}\label{eq:consistent_scribble}
X^{\text{scribbled}}_D \leftarrow \left(\text{clip}_{[-\frac{1}{2},\frac{1}{2}]}\left(X^{\text{scribbled}}_D\oslash M-X_Q\right)+X_Q\right)\odot M.
\end{equation}
The intermediate result is a scribbled image that is consistent with the compressed input code, like the left of the middle pair of images in Fig.~\ref{fig:editing_teaser}. The user then has the option of translating, resizing or rotating the augmented content using arrow buttons, while consistency is re-enforced automatically after each of these operations. Next, the user initiates the optimization process, traversing the $z$ space in an attempt to find the image $\hat{x}$ that is closest to the desired consistent scribble, while lying on the learned manifold of perceptually plausible images.
\paragraph{Imprinting}
This tool enables a user to enforce imported graphical content on the output, either from within the edited image or from an external one. The user first selects the desired content to import, and then marks a bounding rectangle on the edited image, to which the desired content is imprinted. The imprinting itself is performed using the same consistency preserving mechanism used for the scribble tools, including the options to modify the imprinted content's location, size and rotation and including the subsequent optimization process over $z$. We propose a special mechanism to adapt this tool for JPEG compression, which operates on $8\times 8$ pixel blocks, making it highly sensitive to small image shifts. We therefore propose an option to automatically find a shifting of the imprinted content, that yields the most consistent imprinting.
\paragraph{Subtle region shifting}
Instead of marking the desired imprinting location and size, a user can choose to imprint content taken from the edited image onto itself. The user can then utilize the shifting, resizing and rotating buttons to modify the the selected content from its original appearance, thus inducing subtle modifications to selected image regions.
\paragraph{Brightness manipulation}
This tools enables increasing or decreasing current local image brightness by a given, adjustable, factor. The specific image locations to be manipulated are indicated using the entire set of Microsoft-Paint-like tools, after switching their functionality into a ``brightness manipulation'' mode, using the color choice button. After marking desired locations to manipulate, optimization over $z$ attempts to satisfy the desired local relative brightness changes, rather than absolute graphical inputs.
\paragraph{Local TV minimization}
Similar to the brightness manipulation variant, this variant of the graphical input tool-set operates by separately minimizing the total variations (TV) in each separate scribble input. Marking the desired regions is done similarly to the brightness manipulation mode. The optimization process would then operate on all pixels in each marked region, attempting to minimize the magnitude of the differences between each pixel and its $8$ neighboring pixels.
\subsection{Manipulating Hue, Saturation and Relative Brightness (HSV)}
In this work we first introduce a way to manipulate the local hue, saturation and brightness attributes, which are mostly determined by the upper left coefficient of the DCT block, corresponding to the low-frequency image content. Therefore there is no point of exploring these attributes in the super-resolution case, where the low-frequency content is strictly determined by the low-resolution input image, and indeed this mechanism was not proposed in \cite{bahat2019explorable_sr}. Similar to the mechanisms described in Sec.~\ref{sec:graphical_input} for embedding graphical user input, a user can utilize $6$ designated buttons to manipulate HSV values, while consistency is automatically reinforced after each button press by recomputing \ref{eq:consistent_scribble}. To complete the manipulation, an optimization process over $z$ is initiated, similar to all other tools in Sec.~\ref{sec:graphical_input}.
\subsection{Desired Dictionary of Patches}
This tool manipulates (target) patches in a desired region to resemble the patches comprising a desired (source) region, either taken from an external image or from a different location in the edited image. To allow encouraging desired textures across regions with different colors, we first remove mean patch values from each patch, in both source and target patches. To reduce computational load, we discard some of the overlapping patches, by using $2$ and $4$ rows strides in the source and target regions, respectively. Once source and target regions are selected, optimizing over $z$ traverses the learned manifold of valid plausible images to minimize the distance between each target patch and its closest source patch.
\paragraph{Ignoring patches' variance}
A variant of this tool allows encouraging desired textures without changing current local variance. To this end, we normalize patches' variance, in addition to removing their mean. Then while optimizing over $z$, we add an additional objective to preserve the original variance of each target patch, while encouraging its (normalized) signal to resemble that of its closest (normalized) source patch.
\subsection{Encouraging Periodicity}
This tool encourages the periodic nature of an image region, across one or two directions determined by a user. The desired period length (in pixels) for each direction can be manually set by the user, or it can be automatically set to the most prominent period length, by calculating local image self-correlation. Periodicity is then encouraged by penalizing for the difference between the image region and its version translated by a single period length, for each desired direction.
\subsection{Random Diverse Alternatives}
This tool allows exploring the image manifold in a random manner, producing $N$ different outputs by maximizing the $L_1$ distance between them in pixel space. These images (or sub-regions thereof) can then serve as a baseline for further editing and exploration.
\paragraph{Constraining distance to current image}
This variant adds the requirement that all $N$ images should be close to the current $\hat{x}$, in terms of $L_1$ distance in pixel space.
